Intracluster stars in simulations with AGN feedback

We use a set of high-resolution hydrodynamical simulations of clusters of galaxies to study the build-up of the intracluster light (ICL), an interesting and likely significant component of their total stellar mass. Our sample of groups and clusters includes AGN feedback and is of high enough resolution to accurately resolve galaxy populations down to the smallest galaxies that are expected to significantly contribute to the stellar mass budget. We describe and test four different methods to identify the ICL in simulations, thereby allowing us to assess the reliability of the measurements. For all of the methods, we consistently find a very significant ICL stellar fraction (~45%) which exceeds the values typically inferred from observations. However, we show that this result is robust with respect to numerical resolution and integration accuracy, remarkably insensitive to changes in the star formation model, and almost independent of halo mass. It is also almost invariant when black hole growth is included, even though AGN feedback successfully prevents excessive overcooling in clusters and leads to a drastically improved agreement of the simulated cluster galaxy population with observations. In particular, the luminosities of central galaxies and the ages of their stellar populations are much more realistic when including AGN. In the light of these findings, it appears challenging to construct a simulation model that simultaneously matches the cluster galaxy population and at the same time produces a low ICL component. We find that intracluster stars are preferentially stripped in a cluster's densest region from massive galaxies that fall into the cluster at z>1. Surprisingly, some of the intracluster stars also form in the intracluster medium inside cold gas clouds that are stripped out of infalling galaxies.

==> MainMacros.tex <==


% environments:
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}

% math fonts:
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\msf}[1]{\mathsf{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}

% style for vectors, matrices, derivatives etc.:
\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\matr}[1]{\boldsymbol{\mathsf{#1}}}
%\newcommand{\tens}[1]{\boldsymbol{\mathsf{#1}}}

\newcommand{\integral}[4]{\int\limits_{#1}\limits^{#2} #3 \,\mathrm{d}#4\,}
\newcommand{\parder}[3][]{\frac{\partial^{#1} {#2}}{\partial {#3}^{#1}}}
\newcommand{\totder}[3][]{\frac{\mrm{d}^{#1} {#2}}{\mrm{d} {#3}^{#1}}}
\newcommand{\p}{\partial}
\newcommand{\e}{\mathrm{e}}
\newcommand{\diff}[2][]{\mrm{d}^{#1}{#2}\,}
\newcommand{\EV}[1]{\left\langle{#1}\right\rangle}

\newcommand{\order}[2]{\mathrm{o}\left({#1}^{#2}\right)}

% naturals,integers,reals:
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}

% functions:
\newcommand{\tr}{\mrm{tr}\,}
\newcommand{\sign}{\mrm{sign}\,}
\newcommand{\pdf}{\mrm{pdf}}
\newcommand{\cdf}{\mrm{cdf}}
\newcommand{\FWHM}{\mrm{FWHM}}
\newcommand{\arsech}{\mrm{arsech}}
\newcommand{\FT}[1]{\mrm{FT}\!\left[#1\right]}
\newcommand{\IFT}[1]{\mrm{IFT}\!\left[#1\right]}

% units:
\newcommand{\cm}{\ensuremath{\mathrm{cm}}}
\newcommand{\km}{\ensuremath{\mathrm{km}}}
\newcommand{\kms}{\ensuremath{\mathrm{km\,s}^{-1}}}

\newcommand{\pc}{\ensuremath{\mathrm{pc}}}
\newcommand{\kpc}{\ensuremath{\mathrm{kpc}}}
\newcommand{\Mpc}{\ensuremath{\mathrm{Mpc}}}
\newcommand{\Gpc}{\ensuremath{\mathrm{Gpc}}}

\newcommand{\yr}{\ensuremath{\mathrm{yr}}}
\newcommand{\Myr}{\ensuremath{\mathrm{Myr}}}

\newcommand{\Msolar}{\ensuremath{\mathrm{M}_\odot}}
%\newcommand{\mag}{\ensuremath{\mathrm{mag}}}

\newcommand{\MHz}{\ensuremath{\mathrm{MHz}}}

\newcommand{\arcsect}{\ensuremath{\mathrm{arcsec}}}
\newcommand{\arcmint}{\ensuremath{\mathrm{arcmin}}}
\newcommand{\degt}{\ensuremath{\mathrm{deg}}}

%\newcommand{\arcsec}{\ensuremath{''}}
%\newcommand{\arcmin}{\ensuremath{'}}
%\renewcommand{\deg}{\ensuremath{^\circ}}

% freq. used symbols:
\newcommand{\rS}{r_\mrm{S}}
\newcommand{\zS}{z_\mrm{S}}
\newcommand{\zL}{z_\mrm{L}}
\newcommand{\wL}{w_\mrm{L}}
\newcommand{\chiL}{\chi_\mrm{L}}
\newcommand{\aL}{a_\mrm{L}}
\newcommand{\rE}{r_\mrm{E}}
\newcommand{\IIorIII}{\ensuremath{\mrm{II}\vee\mrm{III}}}

\def\21cm{\mbox{21-cm}} 

\newcommand{\clight}{\ensuremath{\mathrm{c}}}
\newcommand{\GNewton}{\ensuremath{\mathrm{G}}}

\newcommand{\Mstellar}{\ensuremath{M_\mrm{stellar}}}
\newcommand{\Mdisc}{\ensuremath{M_\mrm{disc}}}
\newcommand{\Mbulge}{\ensuremath{M_\mrm{bulge}}}
\newcommand{\Sdisc}{\ensuremath{\Sigma_\mrm{disc}}}
\newcommand{\Sbulge}{\ensuremath{\Sigma_\mrm{bulge}}}
\newcommand{\rsdisc}{\ensuremath{r_\mrm{s\,disc}}}
\newcommand{\rsbulge}{\ensuremath{r_\mrm{s\,bulge}}}
\newcommand{\reffdisc}{\ensuremath{r_\mrm{e\,disc}}}
\newcommand{\reffbulge}{\ensuremath{r_\mrm{e\,bulge}}}
\newcommand{\rEinstein}{r_\mrm{E}}


\newcommand{\Ms}{M_\mathrm{s}}
\newcommand{\rs}{r_\mathrm{s}}
\newcommand{\rc}{r_\mathrm{c}}

\newcommand{\DM}{D_\mrm{M}}
\newcommand{\PI}{\mathbb{P}^\mrm{I}}

\newcommand{\zlim}{\ensuremath{z_\text{lim}}}
\newcommand{\Llim}{\ensuremath{L_\text{lim}}}
\newcommand{\mlim}{\ensuremath{m_\text{lim}}}


%\def\simlt{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
%\def\simgt{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}

% % for Latex Macros
% \newcommand{\AddPartToLof}[1]{\addtocontents{lof}{\protect\vspace{0.4cm}}
% \addtocontents{lof}{\protect\begin{center}}
% \addtocontents{lof}{\bfseries{#1}} 
% \addtocontents{lof}{\protect\end{center}}
% \addtocontents{lof}{\protect\vspace{0.4cm}}}
% 
% \newcommand{\AddPartToLot}[1]{\addtocontents{lot}{\protect\vspace{0.4cm}}
% \addtocontents{lot}{\protect\begin{center}}
% \addtocontents{lot}{\bfseries{#1}} 
% \addtocontents{lot}{\protect\end{center}}
% \addtocontents{lot}{\protect\vspace{0.4cm}}}


% \DeclareMathAlphabet{\mymath}{U}{eus}{m}{n}
% 	
% \newcommand{\parHM}{\paragraph{}}
% 
% \def\plotone#1{\centering \leavevmode
% \epsfxsize=0.50\columnwidth \epsfbox{#1}}
% \def\plottwo#1#2{\centering \leavevmode
% \epsfxsize=.50\columnwidth \epsfbox{#1} \hfil
% \epsfxsize=.50\columnwidth \epsfbox{#2}}
% \def\plotthree#1#2#3{\centering \leavevmode
% \epsfxsize=.30\columnwidth \epsfbox{#1} \hfil
% \epsfxsize=.30\columnwidth \epsfbox{#2} \hfil
% \epsfxsize=.30\columnwidth \epsfbox{#3} \hfil}
% 
% 
% \def\spose#1{\hbox to 0pt{#1\hss}}
% 
% 
% 
% \newcommand{\myhline}[1]{
% \setlength{\unitlength}{1mm}
% \linethickness{0.1mm}
% \begin{picture}(#1,0)
% \put(0,0){\line(1,0){#1}}
% \end{picture}
% }
% 


